Weak Keys and Cryptanalysis of a Cold War Block Cipher

T-310 is a cipher that was used for encryption of governmental communications in East Germany during the final years of the Cold War. Due to its complexity and the encryption process,there was no published attack for a period of more than 40 years until 2018 by Nicolas T. Courtois et al. in [10]. In this thesis we study the so called 'long term keys' that were used in the cipher, in order to expose weaknesses which will assist the design of various attacks on T-310.

==> Slide/Slide.tex <==
\chapter{Slide Attack on T-310}

In this chapter, we perform a slide attack on T-310 which is based on the three assumptions below:

\begin{enumerate}
\item The attacker using a decryption oracle attack, described in [], obtains access to $73\%$ of the values $a_i \myeq u_{127\cdot i, \alpha}$, where $i=1,2,3,\cdots$.
\item We recall that the key bits are repeated every 120 rounds. The attacker chooses an IV at random and creates several other IV's which differ by clocking the IV LFSR backwards by $120 \cdot s$ steps, for some integer $s$.
\item The attacker is able to identify whether the internal states are identical,\newline i.e. $u_{0,1-36}=u^{'}_{120\cdot s,1-36}=$ 0xC5A13E396.
\end{enumerate}
Our attack proceeds as follows:\\
Based on the above assumptions, we let $s=127$ and we choose our ciphertexts that are produced with IV to have 5 characters length and those produced with IV', which differs by clocking the IV LFSR backwards by $120 \cdot 127$ steps, to have 1205 characters length. We chose this specific length for our ciphertexts such that after the $120 \cdot 127$ steps, the $5 \cdot 13 = 65$ bits $u_{a \cdot i}$ produced for the encryption of at least 5 characters have an overlap on the secret key bits and IV bits.\\
As mentioned in the assumptions above, we obtain access to $73\%$ of the bits $u_{a \cdot i}$. So for two encryptions that used IV and IV', respectively, we will obtain access to $0.73 \cdot 0.73 \cdot 65 = 35$ values $u_{a \cdot i}$ and $u^{'}_{a \cdot i}$ at the same positions $i$.\\
Then we can conclude that the two states are identical, i.e. $u_{0,1-36}=u^{'}_{120\cdot 127,1-36}=$ 0xC5A13E396, if all 35 bits $u_{a \cdot i}$ and 35 bits $u^{'}_{a \cdot i}$ at the same positions $i$ are exactly the same.\\
In the final step of our attack, we exploit this fact and the fact that the long term key, for example a key that satisfies the conditions of Theorem 3.6, has a linear property for 8 rounds that involves IV and key bits (in our case s1) to construct 8 parity equations in order to recover 8 bits of the secret key.
